Unsupervised Melody-Guided Lyrics Generation

Automatic song writing is a topic of significant practical interest. However, its research is largely hindered by the lack of training data due to copyright concerns and challenged by its creative nature. Most noticeably, prior works often fall short of modeling the cross-modal correlation between melody and lyrics due to limited parallel data, hence generating lyrics that are less singable. Existing works also lack effective mechanisms for content control, a much desired feature for democratizing song creation for people with limited music background. In this work, we propose to generate pleasantly listenable lyrics without training on melody-lyric aligned data. Instead, we design a hierarchical lyric generation framework that disentangles training (based purely on text) from inference (melody-guided text generation). At inference time, we leverage the crucial alignments between melody and lyrics and compile the given melody into constraints to guide the generation process. Evaluation results show that our model can generate high-quality lyrics that are more singable, intelligible, coherent, and in rhyme than strong baselines including those supervised on parallel data.

==> 02-background.tex <==
\section{Background: Melody-Lyrics Alignment}
Music information researchers have found that it is the duration of music notes, not the pitch values that a play significant role in melody-lyric alignment \cite{nichols2009relationships, dzhambazov2017knowledge}. Most intuitively, one ore more music notes should strictly align with one or more syllables in the lyrics. Besides, the segmentation of lyrics should match the segmentation of music phrases for better breathability \cite{watanabe2018melody}. In addition, \citet{nichols2009relationships} find out that there is a correlation between syllable stresses and note durations for better singing rhythm. Namely, shorter note durations are more likely to be associated with unstressed syllables, while longer durations are more likely to be associated with stressed syllables. 

Despite the intuitiveness of the aforementioned alignments, experimental results show that existing lyric generators which are already trained on melody-lyrics aligned data, surprisingly often ignore these fundamental rules and tend generate songs with poor singability. We on the other hand propose to impose such rules at inference time and compile the given melody into constraints to guide lyric generation. Without losing flexibility, we introduce a soften factor to adjust the strength of the constraints.

==> 02-related.tex <==


\section{Related Work}

\subsection{Melody Constrained Lyrics Generation}
Existing works on melody-to-lyrics (M2L) generation mostly focus on the sentence level. For example,
\citet{watanabe2018melody, lee2019icomposer, chen2020melody} train RNNs or LSTMs for such cross-modal alignment, where the input is usually a short piece of melody and output a line of lyrics. Recently,
\citet{sheng2021songmass} propose SongMASS to compose music at the song-level. Specifically, they train a transformer-based model that uses separate encoders and decoders for each modality (lyric or melody) and adopt cross attention to learn the melody-lyrics correlation. However, they all require sizable aligned cross-modal data to train on, and yet the availability of such paired data is extremely limited and the cost of training from scratch is extremely high. Previous works either manually collect a small amount of (usually a few thousand) melody-lyrics pairs \cite{watanabe2018melody, lee2019icomposer}, or use the only publicly available paired data \cite{yu2021conditional} in which the lyrics are pre-tokenized at the syllable level. The loss of word-level integrity in the training data will result in unsatisfactory outputs, which we will show in the generated results in later sections. Our proposed model on the other hand does not require any paired cross-modal data, and is trained on a uni-modal lyrics dataset. Such adaptation also enables us to build upon the powerful massively pre-trained language models such as Bart \cite{lewis2019bart} and GPT-2 \cite{radford2019language} to generate more fluently and coherently.

%Rap generation \cite{xue2021deeprapper} not covered.
 
\subsection{Text Generation with Hierarchical Planning}
Hierarchical generation frameworks are shown to improve consistency over sequence-to-sequence generation frameworks in other creative writing tasks such as story generation \cite{fan2018hierarchical, yao2019plan}. Recently, a similar planning-based scheme is adopted to poetry generation \cite{tian2022zero} to circumvent the lack of poetry data. We on the other hand equip \ModelName{} with the ability to comply with a provided topic via such content planning. To the best of our knowledge, we are the first to propose to add control over the content in the automatic songwriting community. 

\subsection{Studies on Melody-Lyrics Correlation}
Music information researchers have found that it is the duration of music notes, not the pitch values that a play significant role in melody-lyric alignment \cite{nichols2009relationships, dzhambazov2017knowledge}. Most intuitively, one music note should not align with two or more syllables, and the segmentation of lyrics should match the segmentation of music phrases for better singability \cite{watanabe2018melody}. In addition, \citet{nichols2009relationships} find out that there is a correlation between syllable stresses and note durations for better singing rhythm. Namely, shorter note durations are more likely to be associated with unstressed syllables, while longer durations are more likely to be associated with stressed syllables. 

Despite the intuitiveness of the aforementioned alignments, our experimental results show that existing lyric generators which are already trained on melody-lyrics aligned data, surprisingly often ignore these fundamental rules and tend generate songs with poor quality. To the best of our knowledge, we are the first to impose such fundamental rules and compile the given melody into constraints to guide lyric generation at inference time. Without losing flexibility, we introduce a soften factor to adjust the strength of the constraints.
